A Real-time Defense against Website Fingerprinting Attacks

Anonymity systems like Tor are vulnerable to Website Fingerprinting (WF) attacks, where a local passive eavesdropper infers the victim's activity. Current WF attacks based on deep learning classifiers have successfully overcome numerous proposed defenses. While recent defenses leveraging adversarial examples offer promise, these adversarial examples can only be computed after the network session has concluded, thus offer users little protection in practical settings. We propose Dolos, a system that modifies user network traffic in real time to successfully evade WF attacks. Dolos injects dummy packets into traffic traces by computing input-agnostic adversarial patches that disrupt deep learning classifiers used in WF attacks. Patches are then applied to alter and protect user traffic in real time. Importantly, these patches are parameterized by a user-side secret, ensuring that attackers cannot use adversarial training to defeat Dolos. We experimentally demonstrate that Dolos provides 94+% protection against state-of-the-art WF attacks under a variety of settings. Against prior defenses, Dolos outperforms in terms of higher protection performance and lower information leakage and bandwidth overhead. Finally, we show that Dolos is robust against a variety of adaptive countermeasures to detect or disrupt the defense.

==> Makefile <==

LATEX=latex

BIBTEX=bibtex
BIBFILE=zhao.bib wf_defense.bib
PAPER= wf_defense

TEXFILES = wf_defense.tex \
	intro.tex \
	back.tex \
	methodology.tex \
	design.tex \
	eval.tex \
	countermeasures.tex \
	advance.tex \
	discussion.tex \
	appendix.tex 
	
EPSFIGS = \

EPSGRAPHS = $(wildcard figures/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) (PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

# $(PAPER).pdf: $(PAPER).dvi
# 	dvipdf $(PAPER).dvi

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out

